Complete Verification via Multi-Neuron Relaxation Guided Branch-and-Bound

State-of-the-art neural network verifiers are fundamentally based on one of two paradigms: either encoding the whole verification problem via tight multi-neuron convex relaxations or applying a Branch-and-Bound (BaB) procedure leveraging imprecise but fast bounding methods on a large number of easier subproblems. The former can capture complex multi-neuron dependencies but sacrifices completeness due to the inherent limitations of convex relaxations. The latter enables complete verification but becomes increasingly ineffective on larger and more challenging networks. In this work, we present a novel complete verifier which combines the strengths of both paradigms: it leverages multi-neuron relaxations to drastically reduce the number of subproblems generated during the BaB process and an efficient GPU-based dual optimizer to solve the remaining ones. An extensive evaluation demonstrates that our verifier achieves a new state-of-the-art on both established benchmarks as well as networks with significantly higher accuracy than previously considered. The latter result (up to 28% certification gains) indicates meaningful progress towards creating verifiers that can handle practically relevant networks.

==> Makefile <==
# Makefile, allowing to
# - compile
# - test
# - clean
# - run in docker
# For details, see targets defined below
#
# USAGE, for example: make pdf

#####################
# REQUIRED PACKAGES #
#####################

# For instructions on how to set up your system to run all commands here, follow
# https://hub.docker.com/repository/docker/ethsrilab/latex-plus

##############
# PARAMETERS #
##############

# main
OUTPUTDIR := lqa-output
NAME := main

# special
NOAPPENDIX := $(NAME)_no_appendix
FULL := $(NAME)_full
OVERFULL := $(NAME)_overfull
GRAY := $(NAME)_gray
ABSTRACT := $(OUTPUTDIR)/abstract.txt

# submission
SUBMISSIONDIR := submission
ZIP := submission.zip

# log
LATEXMKDIR := $(OUTPUTDIR)/latexmk
LOG := $(OUTPUTDIR)/$(NAME).log
SHORTLOG := $(OUTPUTDIR)/$(NAME)-short.log

LOGFILES := *.aux *.bbl *.log *.bcf  *.blg *.lot *.toc *.swp *.gz *.out *.ttt *.fls *.fdb_latexmk

# scripts

SCRIPTDIR := lqa/scripts

#############
# COMPILING #
#############

LATEXSCRIPT = ./lqa/latex.sh
LATEX := $(LATEXSCRIPT) $(NAME).tex $(LATEXMKDIR)

##########
# OTHERS #
##########

NOAPPENDIXCONFIG := headers/config/noappendix.config
SHOWOVERFULLCONFIG := headers/config/showoverfull.config

########
# PDFS #
########

.DEFAULT_GOAL := pdf-full

.PHONY: pdf-full
pdf-full:
	@echo "\n> COMPILING pdf..."
	$(LATEX)
	@cp $(LATEXMKDIR)/$(NAME).pdf $(OUTPUTDIR)/$(FULL).pdf
	@cp $(LATEXMKDIR)/$(NAME).bbl $(OUTPUTDIR) || true
	@cp $(LATEXMKDIR)/$(NAME).log $(LOG)

.PHONY: pdf-appendix
pdf-appendix: pdf-full
	python3 $(SCRIPTDIR)/pages.py --action appendix

# generate labels into the appendix
.PHONY: appendix-labels
appendix-labels: pdf-full
	cat lqa/other/appendix-labels-loader-1.tex > appendix-labels-loader.tex
	cat $(LATEXMKDIR)/appendix.aux >> appendix-labels-loader.tex
	cat lqa/other/appendix-labels-loader-2.tex >> appendix-labels-loader.tex

# generate PDF without the appendix, but with correct labels into the appendix
.PHONY: pdf-no-appendix
pdf-no-appendix: appendix-labels
	make clean
	touch $(NOAPPENDIXCONFIG)
	$(LATEX)
	@cp $(LATEXMKDIR)/$(NAME).pdf $(OUTPUTDIR)/$(NOAPPENDIX).pdf
	make clean # cleanup

.PHONY: pdf-overfull
pdf-overfull:
	@echo "\n> COMPILING OVERFULL pdf..."
	make clean
	touch $(SHOWOVERFULLCONFIG)
	$(LATEX)
	@cp $(LATEXMKDIR)/$(NAME).pdf $(OUTPUTDIR)/$(OVERFULL).pdf
	make clean # cleanup

.PHONY: pdf-gray
pdf-gray: pdf-full
	@echo "\n> Producing GRAYSCALE version to $(OUTPUTDIR)/$(GRAY).pdf..."
	gs -sOutputFile=$(OUTPUTDIR)/$(GRAY).pdf -sDEVICE=pdfwrite -sColorConversionStrategy=Gray -dProcessColorModel=/DeviceGray -dCompatibilityLevel=1.4 -qQUIET -dNOPAUSE -dBATCH $(OUTPUTDIR)/$(FULL).pdf

.PHONY: pdf-all
pdf-all: cleanall pdf-appendix pdf-no-appendix pdf-overfull pdf-gray pdf-full


# build full pdf but also create synctex files
.PHONY: pdf-full-sync
pdf-full-sync: LATEX += "-synctex=1"
pdf-full-sync: pdf-full
	@cp $(LATEXMKDIR)/$(NAME).synctex.gz $(OUTPUTDIR)/$(FULL).synctex.gz || true


# produce better log files
.PHONY: log
log: pdf-full
	pplatex -i $(LOG) > $(SHORTLOG)


###############
# CONVENIENCE #
###############

.PHONY: check
check: pdf-full log
	python3 $(SCRIPTDIR)/checks.py

.PHONY: text
text: pdf-full
	pdftotext $(OUTPUTDIR)/$(FULL).pdf -raw $(OUTPUTDIR)/$(FULL).txt
	sed -z -i 's/-\n//g' $(OUTPUTDIR)/$(FULL).txt
	sed -z -i 's/\n/ /g' $(OUTPUTDIR)/$(FULL).txt

.PHONY: all
all: pdf-all check log

#########
# CLEAN #
#########

.PHONY: clean
clean:
	@echo "\n> CLEANING temporary files..."
	rm -f $(LOGFILES) || true
	rm -r -f $(LATEXMKDIR) || true
	rm -r -f $(OUTPUTDIR)/script-logs/*.log* || true
	rm -f headers/config/*.config

# make cleanall: remove all produced files
.PHONY: cleanall
cleanall: clean
	@echo "\n> CLEANING PDFs..."
	rm -f *.pdf || true
	cd $(OUTPUTDIR) && rm -f $(LOGFILES) || true
	rm -f $(OUTPUTDIR)/*.pdf || true
	rm -r -f $(SUBMISSIONDIR) || true
	rm -f appendix-labels-loader.tex
	rm -f $(ABSTRACT)

##############
# SUBMISSION #
##############

.PHONY: abstract
abstract:
	python3 $(SCRIPTDIR)/abstract.py

.PHONY: submission-files
submission-files: cleanall abstract pdf-full pdf-appendix pdf-no-appendix

.PHONY: submission
submission: submission-files check
	@echo "\n> PREPARING submission in directory $(SUBMISSIONDIR)..."
	rm -r -f $(SUBMISSIONDIR)
	mkdir $(SUBMISSIONDIR)
	cp $(OUTPUTDIR)/*.pdf $(SUBMISSIONDIR)
	cp $(ABSTRACT) $(SUBMISSIONDIR)
	cp $(OUTPUTDIR)/*.bbl $(SUBMISSIONDIR)

.PHONY: zip-no-appendix
zip-no-appendix: submission
	@rm -f $(SUBMISSIONDIR)/$(ZIP)
	make pdf-no-appendix # update output, prepare appendix labels
	touch $(NOAPPENDIXCONFIG) # ensure appendix is not included when compiling again
	zip --quiet -r $(SUBMISSIONDIR)/$(ZIP) . -x /.git* /$(OUTPUTDIR)* /$(SUBMISSIONDIR)/*.zip
	make clean

.PHONY: zip-full
zip-full: submission
	@rm -f $(SUBMISSIONDIR)/$(ZIP)
	make pdf-full # update output
	# README_publisher.md is wrong in this case
	zip --quiet -r $(SUBMISSIONDIR)/$(ZIP) . -x /.git* /$(OUTPUTDIR)* /$(SUBMISSIONDIR)/*.zip README_publisher.md


#########
# ARXIV #
#########

.PHONY: arxiv-files
arxiv-files: clean
	# clean up outdated directories
	rm -rf arxiv ._arXiv

	# create clean directory
	arxiv_latex_cleaner .
	# rename directory
	mv ._arXiv arxiv

	# copy bbl file
	make pdf-full
	cp $(OUTPUTDIR)/*.bbl ./arxiv

	# cleanup
	rm -f arxiv/Makefile arxiv/README.md arxiv/README_publisher.md

.PHONY: arxiv-check
arxiv-check: pdf-full arxiv-files
	# create pdf
	cd arxiv && latexmk -pdf -interaction=nonstopmode $(NAME).tex

	# check resulting pdf
	# requires pdfdiff: https://github.com/cascremers/pdfdiff
	echo "Differences between two PDFs:"
	pdfdiff --diffviewer diff $(OUTPUTDIR)/$(FULL).pdf ./arxiv/$(NAME).pdf

.PHONY: arxiv
arxiv: arxiv-files
	zip -r $(OUTPUTDIR)/arxiv.zip arxiv

##########
# DOCKER #
##########

DOCKER-CMD := ./lqa/docker.sh


PAPERDIR := $$(pwd)
IMAGE := ethsrilab/latex-plus:version-4.0
CONTAINER := latex-plus-container
RUN := $(DOCKER-CMD) run \
		-it \
		--name $(CONTAINER) \
		--workdir="/paper" \
		-v $(PAPERDIR):/paper \
		$(IMAGE)

# launch a docker container using the image, which will provide a shell in the container
.PHONY: docker-run
docker-run: clean-container
	$(RUN)

# check for updates and remove the created docker container
.PHONY: clean-container
clean-container:
	$(DOCKER-CMD) pull $(IMAGE)
	$(DOCKER-CMD) rm /$(CONTAINER) 2>/dev/null || true

# all above commands, run in docker
.PHONY: docker-all
docker-all: clean-container
	$(RUN) make all

.PHONY: docker-pdf-full
docker-pdf-full: clean-container
	$(RUN) make pdf-full

.PHONY: docker-pdf-full-sync
docker-pdf-full: clean-container
	$(RUN) make pdf-full-sync

.PHONY: docker-pdf-appendix
docker-pdf-appendix: clean-container
	$(RUN) make pdf-appendix

.PHONY: docker-pdf-no-appendix
docker-pdf-no-appendix: clean-container
	$(RUN) make pdf-no-appendix

.PHONY: docker-pdf-overfull
docker-pdf-overfull: clean-container
	$(RUN) make pdf-overfull

.PHONY: docker-pdf-gray
docker-pdf-gray: clean-container
	$(RUN) make pdf-gray

.PHONY: docker-pdf-all
docker-pdf-all: clean-container
	$(RUN) make pdf-all

.PHONY: docker-submission
docker-submission: clean-container
	$(RUN) make submission

.PHONY: docker-check
docker-check: clean-container
	$(RUN) make check

.PHONY: docker-text
docker-text: clean-container
	$(RUN) make text

.PHONY: docker-zip
docker-zip: clean-container
	$(RUN) make zip

.PHONY: docker-zip-no-appendix
docker-zip-no-appendix: clean-container
	$(RUN) make zip-no-appendix

.PHONY: docker-abstract
docker-abstract: clean-container
	$(RUN) make abstract

.PHONY: docker-arxiv
docker-arxiv: clean-container
	$(RUN) make arxiv

.PHONY: docker-arxiv-check
docker-arxiv-check: clean-container
	$(RUN) make arxiv-check


==> acknowledgements.tex <==
\section{Acknowledgments}
\cf{Remove for ICLR}
First and foremost, I want to thank Mark Müller for insightful discussions on technical details, helpful feedback, and being a very supportive supervisor.
Next, a big thank you goes to Nikola Jovanovic for contributing a key part of the implementation. 
Lastly, I want to thank Prof. Dr. Martin Vechev for offering me the opportunity to work on this project and providing the support system to make it successful. 

==> figures/lqa/inkscape-header.tex <==
% Description: Convenience header for usage with inkscape
%
% Usage:
% - Open inkscape
% - Extensions -> TexText
% - Select this header as "Preamble File"
%
% Configure:
% - Comment out the appropriate packages (depending on your template)

%%%%%%%
% ACM %
%%%%%%%
% Conferences with this template
% - PLDI: Conference on Programming Language Design and Implementation
% - POPL: Principles of Programming Languages
% - CCS: Conference on Computer and Communications Security

% \usepackage[tt=false, type1=true]{libertine}
% \usepackage[libertine]{newtxmath}
% \usepackage[T1]{fontenc}

%%%%%%%%%%%%%%%%%%%%%
% ACM with beramono %
%%%%%%%%%%%%%%%%%%%%%
% has a nice monospace font

\usepackage[tt=false, type1=true]{libertine}
\usepackage[libertine]{newtxmath}
\usepackage[scaled=0.8]{beramono} % necessary for nice font in code
\usepackage[T1]{fontenc}

%%%%%%%%%%%%%%%%%
% IEEE standard %
%%%%%%%%%%%%%%%%%
% Conferences with this template:
% - S&P: Symposium on Security and Privacy

% \usepackage{mathptmx}
% \usepackage[T1]{fontenc}

%%%%%%%%%%%%%%%%%%%%%%
% IEEE no times math %
%%%%%%%%%%%%%%%%%%%%%%
% has nicer math

% \usepackage{times}
% \usepackage[T1]{fontenc}


==> headers/header-lqa.tex <==
%%%%%%%%%%%%%%%%%%%
%    PACKAGES     %
%%%%%%%%%%%%%%%%%%%

\usepackage[utf8]{inputenc} % enable UTF-8
\usepackage{lipsum} % write pseudo text

% Why `\usepackage[T1]{fontenc}'?
% https://tex.stackexchange.com/questions/664/why-should-i-use-usepackaget1fontenc
% If you don't use \usepackage[T1]{fontenc},
% - Words containing accented characters cannot be automatically hyphenated,
% - You cannot properly copy-and-paste such words from the output (DVI/PS/PDF),
% - Characters like the pipe sign, less than and greater sign give unexpected
%   results in text.
\usepackage[T1]{fontenc}


%%%%%%%%%%%%%%%%%
% BOOLEAN FLAGS %
%%%%%%%%%%%%%%%%%
\usepackage{etoolbox}
\newbool{includeappendix}
\setbool{includeappendix}{true}

%%%%%%%%%%%%%%%%%%%
% REQUIRED INPUTS %
%%%%%%%%%%%%%%%%%%%

% mark overfull boxes
\input{headers/lqa/overfull}

% comments
\input{headers/lqa/comments}

%%%%%%%%%%%%%%%%%%%
% OPTIONAL INPUTS %
%%%%%%%%%%%%%%%%%%%

% abbreviations
% \input{headers/lqa/abbreviations}

% acronyms
\input{headers/lqa/acronyms}

% subfigures
% \input{headers/lqa/subfigures}

% colors
% \input{headers/lqa/colors}

% listing
\input{headers/lqa/listing}

% clever references
%
% should load last (e.g., after listings) to ensure correct interaction with
% other packages
\input{headers/lqa/references}

% tikz
% \input{headers/lqa/tikz}




==> headers/lqa/abbreviations.tex <==
% Description: This file defines commands for common abbreviations
%
% Usage: \input{headers/lqa/abbreviations}

% The Backslash between `.` and ` ` is needed to ensure the white-space is an
% inter-word space, not a inter-sentence space.
%
% Details:
% - https://tex.stackexchange.com/questions/2229/is-a-period-after-an-abbreviation-the-same-as-an-end-of-sentence-period
% - https://stackoverflow.com/questions/2024338/latex-sometimes-puts-too-much-or-too-little-space-after-periods/2024341

\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }
\newcommand{\etc}{etc.}
\newcommand{\cp}{{cp.\ }}
\newcommand{\nth}[1]{\ensuremath{#1^\text{th}}}
\newcommand{\wrt}{{w.r.t.\ }}

==> headers/lqa/colors.tex <==
% Description: This file contains a few useful colors.
%
% Usage: You may need to comment out the usepackage command below, if they
% conflict with your conference template


%%%%%%%%%
% SETUP %
%%%%%%%%%
% import relevant packages

% Comment out the following line in case of error "Option clash for package color"
\usepackage[usenames, dvipsnames]{color} % for textcolor
\usepackage{xcolor} % for definecolor


%%%%%%%%%%%%%%%%%%%%%%
%  MATPLOTLIB COLORS %
%%%%%%%%%%%%%%%%%%%%%%


% blue
\definecolor{my-full-blue}{HTML}{1F77B4}
%\definecolor{blue}{RGB}{31,119,180} 

% orange
\definecolor{my-full-orange}{HTML}{FF7F0E}
%\definecolor{orange}{RGB}{255,127,14}

% green
\definecolor{my-full-green}{HTML}{2CA02C}
%\definecolor{green}{RGB}{44,160,44}

% red
\definecolor{my-full-red}{HTML}{d62728}
%\definecolor{red}{RGB}{214,39,40}

% purple
\definecolor{my-full-purple}{HTML}{9467bd}
%\definecolor{purple}{RGB}{148,103,189}

% brown
\definecolor{my-full-brown}{HTML}{8c564b}
%\definecolor{brown}{RGB}{140,86,75}

% pink
\definecolor{my-full-pink}{HTML}{e377c2}
%\definecolor{pink}{RGB}{227,119,194}

% gray
\definecolor{my-full-gray}{HTML}{7f7f7f}
%\definecolor{gray}{RGB}{127,127,127}

% olive
\definecolor{my-full-olive}{HTML}{bcbd22}
%\definecolor{olive}{RGB}{188,189,34}

% cyan
\definecolor{my-full-cyan}{HTML}{17becf}
%\definecolor{cyan}{RGB}{23,190,207}

% lighter shades
\colorlet{my-blue}{my-full-blue!30}
\colorlet{my-orange}{my-full-orange!30}
\colorlet{my-green}{my-full-green!30}
\colorlet{my-red}{my-full-red!30}
\colorlet{my-purple}{my-full-purple!30}
\colorlet{my-brown}{my-full-brown!30}
\colorlet{my-pink}{my-full-pink!30}
\colorlet{my-gray}{my-full-gray!30}
\colorlet{my-olive}{my-full-olive!30}
\colorlet{my-cyan}{my-full-cyan!30}

%%%%%%%%%%%%%%%%%%%%%%
%  PROJECT-SPECIFIC  %
%%%%%%%%%%%%%%%%%%%%%%
% add project-specific colors here

==> headers/lqa/csvsimple.tex <==
% Description: This file enables displaying csv tables
%
% Usage: \input{headers/lqa/csvsimple}

\usepackage{csvsimple}

% EXAMPLE USAGE

% \begin{table}
% 	\begin{tabular}{ll}
% 		A & B \\
% 		\hline
% 		\csvreader[%
% 			head to column names,
% 			late after line=\\,
% 			separator=semicolon
% 		]{algorithms.csv}{}{%
% 			\a & \b
% 		}
% 	\end{tabular}
% 	\caption{Caption.}
% 	\label{tab:label}
% \end{table}

==> headers/lqa/headings.tex <==
% Description: This file defines headings
%
% Usage: \input{headers/lqa/headings}

\makeatletter

% for IEEE:
% replace trailing : by trailing .
\def\@IEEEsectpunct{.\ }

% Definition for paragraphs, handling spacing correctly
% https://tex.stackexchange.com/questions/31780/where-can-i-find-help-files-or-documentation-for-commands-like-startsection-fo
% http://joshua.smcvt.edu/latex2e/bs-at-startsection.html
\def\para{\@startsection%
	{paragraph}% 
	{4}% level
	{0\parindent}% indent
	{0.6ex plus 0.1ex minus 0.1ex}% beforeskip
	{0ex}% afterskip
	{\normalfont\normalsize\itshape\bfseries}% style
	*% do not number
}%

\makeatother


% Alternatively: Define \para in terms of \paragraph
% \newcommand{\para}[1]{\paragraph{#1.}}

==> headers/lqa/subfigures.tex <==
% Description: This file introduces a subfigure which correctly aligns
% captions
%
% Usage:
% - \input{headers/lqa/subfigures}
% - You may need to comment out the usepackage command below in case of
%   conflicts

% EXAMPLE USAGE:
%
% \begin{figure}
% 	\centering
% 	\mysubfigure[0.49\linewidth]{
% 		\centering
% 		Content of subfigure 1
% 	}{Caption of subfigure\label{fig:subfig1}}
% 	\mysubfigure[0.49\linewidth]{
% 		\centering
% 		Content of subfigure 2
% 	}{Caption of subfigure\label{fig:subfig2}}
% 	\caption{An example of subfigures.}
% 	\label{fig:subfigures}
% \end{figure}

%%%%%%%%%%%%%%
% USEPACKAGE %
%%%%%%%%%%%%%%
\usepackage{subcaption}

%%%%%%%%%%%
% COMMAND %
%%%%%%%%%%%

\newcommand{\mysubfigure}[3][\linewidth]{\subcaptionbox{#3}[#1]{
	\begin{minipage}{#1}
		% uses minipage to prevent unexpected interactions,
		% e.g., for align
		#2
	\end{minipage}
}}


==> headers/lqa/tikz.tex <==
% Description: This file contains a few useful tikz libraries.
%
% Usage: \input{headers/lqa/tikz}

%%%%%%%%%
% SETUP %
%%%%%%%%%
% import relevant package
\usepackage{tikz}

%%%%%%%%%%%%%%%%%%%%%%
%  PROJECT-SPECIFIC  %
%%%%%%%%%%%%%%%%%%%%%%
% adapt the following list of libraries as required

\usetikzlibrary{arrows}
\usetikzlibrary{automata}
\usetikzlibrary{calc}
\usetikzlibrary{backgrounds}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{fit}
\usetikzlibrary{patterns}
\usetikzlibrary{positioning}
\usetikzlibrary{shadows}
\usetikzlibrary{shapes}
\usetikzlibrary{shapes.geometric}








==> lqa/scripts/tests/abstract/header.tex <==
%%%%%%%%%%%%%%%%%
% ABBREVIATIONS %
%%%%%%%%%%%%%%%%%


\newcommand{\eg}{e.g., }
\newcommand{\tool}[0]{\emph{Sometool}\xspace}


==> lqa/scripts/tests/header/cmd.tex <==
abc

\newcommand{\cmd}[0]{cmd}


==> lqa/scripts/tests/header/package.tex <==
abc

\usepackage{abc}


==> lqa/scripts/tests/helpers/main.tex <==
x1
% x2
x3 % x4
x5 \% x6
x7\begin{comment}
x8
\end{comment}x9
x10


==> lqa/scripts/tests/hyphenation/check.tex <==
These occurrences should be fine:

We compute it in constant-time successfully.
We achieve state-of-the-art results.
May hyphenated words may occur at sentence-end?
Hyphenated words may occur at sentence-end.
Hyphenated words may occur at sentence-end!
single-occurrence
occurrence-one occurrence-two
multiple real-worlds

These occurrences should be reported:

We should not write constant time here.
single occurrence
We should not write state-of-the art.


==> lqa/scripts/tests/hyphenation/parse.tex <==
We compute it in constant-time successfully.

We achieve state-of-the-art results.

May hyphenated words may occur at sentence-end?

Hyphenated words may occur at sentence-end.

Hyphenated words may occur at sentence-end!

single-occurrence

occurrence-one occurrence-two

multiple real-worlds

should ignore this: $a-b$

==> lqa/scripts/tests/merge_msgs/merge_msgs.tex <==
Hello world

<<<<<<< HEAD
this is some content to mess with
content to append

=======
totally different content to merge later
>>>>>>> 0489das287d4639d049dddas
that's it


==> lqa/scripts/tests/parse_latex/parser-body.tex <==
\section{My section}

Hello world! This is just an example text that spans multiple lines,
which we can hopefully parse correctly. Even the \emph{third} line should
work if the developers did a good job.

Also a second paragraph goes here. We present \systemname, the first tool
to automatically perform great tasks.

\paragraph{First step} Read this fancy paragraph that even contains
math $x < 3$ in it! There is some continuation of this text, which
should be merged together with part of the text that comes before
the inlined math.

The following formula
\[
    e = mc^2    
\]
is inlined into a sentence.

\begin{figure}
    \centering
    This is a figure content
    \caption{This is a caption}\label{fig:sample-label}
\end{figure}

\begin{enumerate}
    \item First item containing \emph{emphasis} in it % and a comment
          and continues here
    \item Second item
\end{enumerate}

==> lqa/scripts/tests/parse_latex/parser-header.tex <==
\usepackage{xcolor} % for definecolor
\usepackage{amsthm, amsmath}

\newcommand{\systemname}[0]{MySystem}
\newcommand{\eg}[1]{\emph{e.g.,~}}


==> lqa/scripts/tests/references/eqref.tex <==
abc \eqref{def}


==> lqa/scripts/tests/references/ref.tex <==
abc \ref{def}


==> lqa/scripts/tests/unreferenced_floats/floats.tex <==
\section{My section}\label{sec:section}
Hello! We are now referencing \cref{fig:example} and also \cref{tab:example}, but nothing else.

\lstinputlisting[caption={Example code.},label=lst:example]{inexistent.java}

\begin{figure}
    Test
    \caption{Some caption}\label{fig:example}
\end{figure}

\begin{table}
    Test
    \caption{Some caption}
    \label{tab:example}
\end{table}

\begin{figure}
    Test
    \caption{Some caption}
    \label{fig:example_missing}
\end{figure}

\begin{table}
    Test
    \caption{Some caption}\label{tab:example_missing}
\end{table}

==> test-section.tex <==
\section{Test Section} \label{sec:test}

Interesting stuff:

\begin{itemize}
	\item Citations are set up already: Turing~\cite{turing1937computable}
	\item You may use UTF-8 characters: ä
	\item Use cref for references: \cref{sec:test}
	\item Reference the appendix: \cref{fig:appendix} in \cref{app:test-appendix}
	\item Use the \texttt{acro} package for acronyms: First usage: \ac{cli}, subsequent usages: \ac{cli}
\end{itemize}

\begin{figure}[t]
	\centering
	\includegraphics[height=2cm]{example-image-a}
	\caption{An example figure caption.}
	\label{fig:example}
\end{figure}

\paragraph{Figures}
See \cref{fig:example} for an example figure.

\lstinputlisting[float=t,caption={Example code.},label=lst:code]{code/example-code.psi}

\paragraph{Listings}
See \cref{lst:code} for an example Listing.

